A Desideratum for Conversational Agents: Capabilities, Challenges, and Future Directions

Recent advances in Large Language Models (LLMs) have propelled conversational AI from traditional dialogue systems into sophisticated agents capable of autonomous actions, contextual awareness, and multi-turn interactions with users. Yet, fundamental questions about their capabilities, limitations, and paths forward remain open. This survey paper presents a desideratum for next-generation Conversational Agents - what has been achieved, what challenges persist, and what must be done for more scalable systems that approach human-level intelligence. To that end, we systematically analyze LLM-driven Conversational Agents by organizing their capabilities into three primary dimensions: (i) Reasoning - logical, systematic thinking inspired by human intelligence for decision making, (ii) Monitor - encompassing self-awareness and user interaction monitoring, and (iii) Control - focusing on tool utilization and policy following. Building upon this, we introduce a novel taxonomy by classifying recent work on Conversational Agents around our proposed desideratum. We identify critical research gaps and outline key directions, including realistic evaluations, long-term multi-turn reasoning skills, self-evolution capabilities, collaborative and multi-agent task completion, personalization, and proactivity. This work aims to provide a structured foundation, highlight existing limitations, and offer insights into potential future research directions for Conversational Agents, ultimately advancing progress toward Artificial General Intelligence (AGI). We maintain a curated repository of papers at: https://github.com/emrecanacikgoz/awesome-conversational-agents.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/abstract_openreview.tex <==
Recent advances in Large Language Models (LLMs) have propelled conversational AI from traditional dialogue systems into sophisticated agents capable of autonomous actions, contextual awareness, and multi-turn interactions with users. 
Yet, fundamental questions about their capabilities, limitations, and paths forward remain open.
This survey paper presents a desideratum for next-generation Conversational Agents—*what has been achieved*, *what challenges persist*, and *what must be done for more scalable systems that approach human-level intelligence*. 
To that end, we systematically analyze LLM-driven Conversational Agents by organizing their capabilities into three primary dimensions: (i) **Reasoning**—logical, systematic thinking inspired by human intelligence for decision making, (ii) **Monitoring**—encompassing self-awareness and user interaction monitoring, and (iii) **Control**—focusing on tool utilization and policy following.
Building upon this, we introduce a novel taxonomy by classifying recent work on Conversational Agents around our proposed desideratum. 
We identify critical research gaps and outline key directions, including **realistic evaluations**, **long-term multi-turn reasoning skills**, **self-evolution capabilities**, **collaborative and multi-agent task completion**, **personalization**, and **proactivity**. 
This work aims to provide a structured foundation, highlight existing limitations, and offer insights into potential future research directions for Conversational Agents, ultimately advancing progress toward Artificial General Intelligence (AGI).


Recent advances in Large Language Models (LLMs) have propelled conversational AI from traditional dialogue systems into sophisticated agents capable of autonomous actions, contextual awareness, and multi-turn interactions with users. 
Yet, fundamental questions about their capabilities, limitations, and paths forward remain open.
This survey paper presents a desideratum for next-generation Conversational Agents—what has been achieved, what challenges persist, and what must be done for more scalable systems that approach human-level intelligence. 
To that end, we systematically analyze LLM-driven Conversational Agents by organizing their capabilities into three primary dimensions: (i) Reasoning—logical, systematic thinking inspired by human intelligence for decision making, (ii) Monitor—encompassing self-awareness and user interaction monitoring, and (iii) Control—focusing on tool utilization and policy following.
Building upon this, we introduce a novel taxonomy by classifying recent work on Conversational Agents around our proposed desideratum. 
We identify critical research gaps and outline key directions, including realistic evaluations, long-term multi-turn reasoning skills, self-evolution capabilities, collaborative and multi-agent task completion, personalization, and proactivity. 
This work aims to provide a structured foundation, highlight existing limitations, and offer insights into potential future research directions for Conversational Agents, ultimately advancing progress toward Artificial General Intelligence (AGI). We maintain a curated repository of papers at: \url{https://github.com/emrecanacikgoz/awesome-conversational-agents}.


==> sections/tables/taxonomy-awareness.tex <==
\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=7.0em,font=\tiny,}{},
            where level=2{text width=4.3em,font=\tiny,}{},
            where level=3{last level, text width=19em,font=\tiny,}{},
            [
                Situation Awareness (\S \ref{sec:awareness}), ver
                [
                    User awareness
                    [
                    {
                    \textbf{User Intention} TODO;\\
                    \textbf{Personality \& Persona} TODO;\\
                    \textbf{User Emotion \& Sentiment} TODO;
                    }
                    ]
                ]
                [
                    Self Awareness
                    [
                    {
                    \textbf{Knowledge Boundary} TODO;\\
                    \textbf{Self-Correction} Self-Refine~\citep{madaan2023sr}{,} \\ Reflexion~\citep{shinn2023reflexion}{,} ETO~\citep{song2024eto}{,} \\ IPR~\citep{xiong2024ipr}{,} AgentRefine~\citep{fu2025agentrefine}{,} \\ Agent-R~\citep{yuan2025agentr};
                    }
                    ]
                ]
                [
                    Environment \\ Awareness
                    [
                    {
                    \textbf{Memory} TODO;\\
                    \textbf{Proactivity} TODO; \\
                    \textbf{Self-Evolution} TODO; \\
                    }
                    ]
                ]
            ]

        \end{forest}
    }

==> sections/tables/taxonomy-basics.tex <==
 v\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=7.0em,font=\tiny,}{},
            where level=2{text width=4.3em,font=\tiny,}{},
            where level=3{last level, text width=19em,font=\tiny,}{},

            [
                Basic Components (\S \ref{sec:core_components}), ver
                [
                    Goal-Oriented
                    [
                    PPTOD~\citep{su-etal-2022-multi-pptod}{,} InstructTOD~\citep{chung-etal-2023-instructtods}{,} \\ SGPTOD~\citep{zhang2023sgptod}{,} \cite{hudecek-dusek-2023-are_llms_tod}{,} \\ FNCTOD~\citep{li2024fnctod}{,} 
                    AutoTOD~\citep{xu2024autotod}{,} \\ \cite{king-flanigan-2024-unsupervised}
                    ]
                ]
                [
                    Open-ended
                    [
                    DialogGPT~\citep{zhang-etal-2020-dialogpt}{,} \\
 BlenderBot~\citep{shuster2022blenderbot}
                    ]
                ]
                [
                    Autonomy
                    [
                    AutoTOD~\citep{xu2024autotod}{,}
                    ]
                ]
                [
                    Reasoning \\ \& Planning
                    [
                    CoT~\citep{wei2022chain}{,} SC~\citep{wang2022sc}{,} \\ Self-Refine~\citep{madaan2023sr}{,} Reflexion~\citep{shinn2023reflexion}{,} \\ ToT~\citep{yao2023tree}{,} ReSpAct~\citep{dongre2024respact}{,} \\ TravelPlanner~\citep{xie2024travelplanner}
                    ]
                ]
            ]

        \end{forest}
    }
    \caption{Taxonomy of Conversational Agents.}
    \label{fig: taxonomy}
\end{figure*}

==> sections/tables/taxonomy-interactivity.tex <==
\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=7.0em,font=\tiny,}{},
            where level=2{text width=4.3em,font=\tiny,}{},
            where level=3{last level, text width=19em,font=\tiny,}{},


            [
                Interactivity (\S \ref{sec:interactivity}), ver
                [
                    State Tracking
                    [
                    IC-DST~\citep{hu2022icdst}{,} LDST~\citep{feng2023ldst}{,} \\ \cite{hudecek-dusek-2023-are_llms_tod}{,} FNCTOD~\citep{li2024fnctod}{,} \\ \cite{king-flanigan-2024-unsupervised};\\
                    ]
                ]
                [
                    Policy Alignment
                    [
                    {
                    TODO;\\
                    }
                    ]
                ]
                [
                    Tool Invocation
                    [
                    {
                    TALM~\citep{parisi2022talm}{,} Toolformer~\citep{schick2023toolformer}{,} \\ ToolAlpaca~\citep{tang2023toolalpaca}{,} Agent-Tuning~\citep{zeng2024agenttuning}{,} \\ Agent-Flan~\citep{chen2024agentflan}{,} xLAM~\citep{zhang2024xlam}{,} \\ ToolAce~\citep{liu2025toolace}{,} Hammer~\citep{lin2025hammer};\\
                    }
                    ]
                ]
                [
                    Multi-Agent \\ \& Concierge
                    [
                    {
                    TODO;\\
                    }
                    ]
                ]
                [
                    Conversational \\ Strategy
                    [
                    {
                    \textbf{Single-Turn} TODO;\\
                    \textbf{Multi-Turn} TODO;\\
                    }
                    ]
                ]
            ]
        \end{forest}
    }


==> sections/tables/taxonomy-ver2.tex <==
% TikZ styles for the diagram
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-orange!60, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[tp]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=5.2em,font=\scriptsize,}{},
            where level=2{text width=5.2em,font=\scriptsize,}{},
            where level=3{text width=7.5em,font=\scriptsize,}{},
            where level=4{text width=8em,font=\scriptsize,}{},
            [
                    Conversational \\ Agents (\S \ref{sec:core_components})
                    [
                        Core Components \\ (\S \ref{sec:tool_integration})
                        [
                            Goal-Oriented \\ Objective
                            [
                                PPTOD{,} InstructTOD{,} SGPTOD{,} InstructTOD{,} Vojtech{,} FNCTOD{,} SGPTOD{,} AutoTOD{,} Brendan
                                , leaf, text width=44.7em
                            ]
                        ]
                        [
                            Open-end Skills
                            [
                                TODO
                                , leaf, text width=44.7em
                            ]
                        ]
                        [
                            Task Autonomy
                            [
                                AutoTOD
                                , leaf, text width=44.7em
                            ]
                        ]
                        [
                            Reasoning{,} \\ Planning \&  Acting
                            [
                                CoT{,} SC{,} Self-refine{,} ReAct{,} Reflexion{,} ToT{,} ReSpAct
                                , leaf, text width=44.7em
                            ]
                        ]
                    ]
                    [
                        Situation \\   Awareness(\S \ref{sec:awareness})
                        [
                            User Awareness
                            [
                                User Intention
                                [
                                    IN3~\citep{shen2024smartcal}{,} https://arxiv.org/pdf/2503.01940 Sec2.2
                                    , leaf, text width=35.7em
                                ]
                            ]
                            [
                             Personality \& Persona
                                [
                                    TODO
                                    , leaf, text width=35.7em
                                ]
                            ]
                            [
                            User Emotion \& \\ Sentiment
                                [
                                    TODO
                                    , leaf, text width=35.7em
                                ]
                            ]
                        ]
                        [
                            Self Awareness
                            [
                                Self Knowledge \\ Boundary
                                [
                                    SMARTCAL~\citep{shen2024smartcal}{,}
                                    CalibratedMath-\emph{k}~\citep{lin2022teaching}{,}
                                    LLM Uncertainty~\citep{xiong2024can}{,} \\
                                    SMART
                                    , leaf, text width=35.7em
                                ]
                            ]
                            [
                                Self Correction
                                [
                                    Self-refine{,} Reflexion{,} ETO{,} IPR{,} AgentRefine{,} Agent-R
                                    , leaf, text width=35.7em
                                ]
                            ]
                        ]
                        [
                            Environment \\ Awareness
                            [
                                External Modules: \\ Memory
                                [
                                    TODO
                                    , leaf, text width=35.7em
                                ]
                            ]
                            [
                               External Events: \\ Proactivity
                                [
                                    TODO
                                    , leaf, text width=35.7em
                                ]
                            ]
                            [
                                External Feedback: \\ Self-Evolution
                                [
                                    TODO
                                    , leaf, text width=35.7em
                                ]
                            ]
                        ]
                    ]
                    [
                        Interactivity(\S \ref{sec:awareness})
                        [
                            Dialogue \\ State-Tracking
                            [
                                IC-DST{,} LDST{,} Vojtech{,} TODO{,} LDST{,} Vojtech{,} Brendan
                                , leaf, text width=44.7em
                            ]
                        ]
                        [
                            Policy Alignment
                            [
                                TODO
                                , leaf, text width=44.7em
                            ]
                        ]
                        [
                            Tool Invocation
                            [
                                TALM{,} Toolformer{,} ToolAlpaca{,} Agent-TUning{,} FireAct{,} Agent-Flan{,} xLAM{,} ToolAce{,} Hammer{,}
                                , leaf, text width=44.7em
                            ]
                        ]
                        [
                            Multi-Agent \& \\ Concierge
                            [
                                TODO
                                , leaf, text width=44.7em
                            ]
                        ]
                        [
                            Conversational \\ Strategy
                            [
                                TODO
                                , leaf, text width=44.7em
                            ]
                        ]

                    ]
                ]

        \end{forest}
    }
    \caption{Taxonomy of Conversational Agents.}
    \label{fig: taxonomy}
\end{figure*}

==> sections/tables/taxonomy-ver3.tex <==
\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=7.0em,font=\tiny,}{},
            where level=2{text width=4.3em,font=\tiny,}{},
            where level=3{last level, text width=19em,font=\tiny,}{},
            [
                Conversational Agents, ver
                [
                    Basic Components (\S \ref{sec:core_components}), ver
                    [
                        Goal-Oriented
                        [
                        PPTOD~\citep{su-etal-2022-multi-pptod}{,} InstructTOD~\citep{chung-etal-2023-instructtods}{,} \\ SGPTOD~\citep{zhang2023sgptod}{,} \cite{hudecek-dusek-2023-are_llms_tod}{,} \\ FNCTOD~\citep{li2024fnctod}{,} AutoTOD~\citep{xu2024autotod}{,} \\ \cite{king-flanigan-2024-unsupervised}{,} CoALM~\citep{acikgoz2025singlemodelmastermultiturn}
                        ]
                    ]
                    [
                        Open-ended
                        [
                        WoW~\citep{dinan2019wow}{,}
                        DialogGPT~\citep{zhang-etal-2020-dialogpt}{,} \\ BlenderBot~\citep{shuster2022blenderbot}
                        BoB~\citep{song-etal-2021-bob}{,} \\
                        DuClarifyDial~\citep{liu-etal-2022-go}{,} PLATO~\citep{bao-etal-2021-plato}
                        ]
                    ]
                    [
                        Autonomy
                        [
                        AutoTOD~\citep{xu2024autotod}{,}
                        ]
                    ]
                    [
                        Reasoning \\ \& Planning
                        [
                        CoT~\citep{wei2022chain}{,} SC~\citep{wang2022sc}{,} \\ Self-Refine~\citep{madaan2023sr}{,} Reflexion~\citep{shinn2023reflexion}{,} \\ ToT~\citep{yao2023tree}{,}Cue-CoT~\citep{wang-etal-2023-cue}{,} \\ ReSpAct~\citep{dongre2024respact}{,} TravelPlanner~\citep{xie2024travelplanner}
                        ]
                    ]
                ]
                [
                    Situation Awareness (\S \ref{sec:awareness}), ver
                    [
                        User awareness
                        [
                        {
                        \textbf{User Intention} INTENT-SIM~\citep{zhang2023clarify}{,}\\ Intention-in-Interaction~\citep{qian2024tell}{,} AwN~\citep{wang2024learning}{,}\\
                        STaR-GATE~\citep{andukuri2024star}{,} AskToAct~\citep{zhang2025asktoact}\\
                        \textbf{Personality \& Persona} BeCand~\citep{lim2023beyond}{,}\\ PAA~\citep{huang2023personalized}{,} CharacterChat~\citep{tu2023characterchat} ...\\ (should check here: \url{https://github.com/Sahandfer/PersonaPaper})\\
                        \textbf{User Emotion \& Sentiment} EmpatheticDialogues~\citep{rashkin-etal-2019-towards} \\ 
                        ESConv~\citep{liu2021towards}{,} D4~\citep{yao-etal-2022-d4}{,} RR~\citep{fu-etal-2023-reasoning} \\
                        ChatCounsel~\citep{liu2023chatcounselorlargelanguagemodels};
                        }
                        ]
                    ]
                    [
                        Self Awareness
                        [
                        {
                        \textbf{Self-Imposed Capability Limit} SMARTAgent~\citep{qian2025smart}{,}\\ MeCo~\citep{li2025adaptive}, KnowSelf~\citep{qiao2025agentic}\\
                        \textbf{Self-Correction} Self-Refine~\citep{madaan2023sr}{,} \\ Reflexion~\citep{shinn2023reflexion}{,} ETO~\citep{song2024eto}{,} \\ IPR~\citep{xiong2024ipr}{,} AgentRefine~\citep{fu2025agentrefine}{,} \\ Agent-R~\citep{yuan2025agentr};
                        }
                        ]
                    ]
                    [
                        Environment \\ Awareness
                        [
                        {
                        \textbf{Modules} FoCus~\citep{jang2022call}{,} DuLeMon~\citep{xu-etal-2022-long}{,} \\ SAFARI~\citep{wang-etal-2023-large};\\
                        \textbf{Proactivity} Proactive DA~\citep{kraus2023improving}{,} CEP~\citep{zhang2024ask}{,} \\ ProactiveAgent~\citep{lu2024proactive}{,} \\
                        \textbf{Evolution} SPDA~\citep{cheng2024autopal}{,} ICE~\citep{qian2024investigate}{,}\\ THEANINE~\citep{ong2024towards} \\
                        }
                        ]
                    ]
                ]
                [
                    Interactivity (\S \ref{sec:interactivity}), ver
                    [
                        State Tracking
                        [
                        IC-DST~\citep{hu2022icdst}{,} LDST~\citep{feng2023ldst}{,} \\ \cite{hudecek-dusek-2023-are_llms_tod}{,} FNCTOD~\citep{li2024fnctod}{,} \\ \cite{king-flanigan-2024-unsupervised}{,} CoALM~\citep{acikgoz2025singlemodelmastermultiturn};\\
                        ]
                    ]
                    [
                        Policy Alignment
                        [
                        {
                        PPO-Off~\citep{ppooffgan};\\
                        }
                        ]
                    ]
                    [
                        Tool Invocation
                        [
                        {
                        TALM~\citep{parisi2022talm}{,} Toolformer~\citep{schick2023toolformer}{,} \\ ToolAlpaca~\citep{tang2023toolalpaca}{,} Agent-Tuning~\citep{zeng2024agenttuning}{,} \\ Agent-Flan~\citep{chen2024agentflan}{,} xLAM~\citep{zhang2024xlam}{,} \\ ToolAce~\citep{liu2025toolace}{,} Hammer~\citep{lin2025hammer};\\
                        AppBench~\citep{wang-etal-2024-appbench}
                        }
                        ]
                    ]
                    [
                        Multi-Agent \\ \& Concierge
                        [
                        {
                        Generative Agents~\citep{generative_agents}{,} CAMEL~\citep{li2023camel}{,} \\ AutoGen~\citep{wu2024autogen}{,} OrchestraLLM~\citep{lee2024orchestrallm};\\
                        }
                        ]
                    ]
                    [
                        Conversational \\ Strategy
                        [
                        {
                        \textbf{Single-Turn} TALM~\citep{parisi2022talm}{,} \\ Toolformer~\citep{schick2023toolformer}{,} ToolAlpaca~\citep{tang2023toolalpaca}{,} \\ xLAM~\citep{zhang2024xlam}{,} Hammer~\citep{lin2025hammer};\\
                        \textbf{Multi-Turn} Agent-Tuning~\citep{zeng2024agenttuning}{,} \\ Agent-Flan~\citep{chen2024agentflan}{,} FNCTOD~\citep{li2024fnctod}{,} \\ ToolAce~\citep{liu2025toolace}{,} AutoTOD~\citep{xu2024autotod}{,} \\  CoALM~\citep{acikgoz2025singlemodelmastermultiturn};\\
                        }
                        ]
                    ]
                ]
            ]
        \end{forest}
    }

==> sections/tables/taxonomy-ver4.tex <==
\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=7.0em,font=\tiny,}{},
            where level=2{text width=4.3em,font=\tiny,}{},
            where level=3{last level, text width=19em,font=\tiny,}{},
            [
                Conversational Agents, ver
                [
                    Reasoning{,} Planning{,} \\ and Acting (\S \ref{sec:core_components}), ver
                    [
                        Complex \\ Reasoning % Planning should be there
                        [
                        CoT~\citep{wei2022chain}{,} SC~\citep{wang2022sc}{,} \\ Self-Refine~\citep{madaan2023sr}{,} Reflexion~\citep{shinn2023reflexion}{,} \\ ToT~\citep{yao2023tree}{,} Cue-CoT~\citep{wang-etal-2023-cue}{,} \\ ReSpAct~\citep{dongre2024respact}
                        ]
                    ]
                    [
                        Tool Usage % Knowledge Injection, RAG: Previously they use Information Retrievel, Rag now tools.
                        [
                        TALM~\citep{parisi2022talm}{,} Toolformer~\citep{schick2023toolformer}{,} \\ ToolAlpaca~\citep{tang2023toolalpaca}{,} Agent-Tuning~\citep{zeng2024agenttuning}{,} \\ Agent-Flan~\citep{chen2024agentflan}{,} FNCTOD~\citep{li2024fnctod}{,} \\ ToolAce~\citep{liu2025toolace}{,} Hammer~\citep{lin2025hammer};\\
                        AppBench~\citep{wang-etal-2024-appbench}
                        ]
                    ]

                    [
                        Policy Following % construct reward, faciliate it is as rubrics
                        [
                        {
                        SGPTOD~\citep{zhang2023sgptod}{,} \cite{hudecek-dusek-2023-are_llms_tod}{,} \\ FlowBench~\citep{xiao2024flowbench}{,}  AutoTOD~\citep{xu2024autotod}{,} \\
                        }
                        ]
                    ]
                    % [
                    %     Knowledge \\ Injection
                    %     [
                    %     WoW~\citep{dinan2019wow}{,}
                    %     BlenderBot~\citep{shuster2022blenderbot} \\
                    %     BoB~\citep{song-etal-2021-bob}{,} 
                    %     PLATO~\citep{bao-etal-2021-plato}
                    %     ]
                    % ]
                ]
                % [   % 
                %     Policy{,} Alignment{,} \& \\ Safety (\S \ref{sec:awareness}), ver
                %     [
                %         Policy \& \\ Instruction \\ Following
                %         [
                %         {
                %         SGPTOD~\citep{zhang2023sgptod}{,} \cite{hudecek-dusek-2023-are_llms_tod}{,} \\ FlowBench~\citep{xiao2024flowbench}{,}  AutoTOD~\citep{xu2024autotod}{,} \\
                %         }
                %         ]
                %     ]
                %     [
                %         Safety
                %         [
                %         {
                %         TODO
                %         }
                %         ]
                %     ]
                % ]
                % [
                %     Context \& Memory (\S \ref{sec:interactivity}), ver
                    
                %     [
                %         Dialogue \\ Memory \\ Management
                %         [
                %         {
                %         TODO
                %         }
                %         ]
                %     ]
                %     [
                %         Knowledge \\ Retrieval
                %         [
                %         {
                %         TODO
                %         }
                %         ]
                %     ]
                % ]
                [
                    Self Awareness (\S \ref{sec:interactivity}), ver
                    [
                        Self-Impose \\ Capability
                        [
                        {
                        SMARTAgent~\citep{qian2025smart}{,}\\ MeCo~\citep{li2025adaptive}, KnowSelf~\citep{qiao2025agentic}
                        }
                        ]
                    ]
                    [
                        Self-Assessment \\ \& Correction
                        [
                        {
                        Self-Refine~\citep{madaan2023sr}{,} Reflexion~\citep{shinn2023reflexion}{,} \\ ETO~\citep{song2024eto}{,} IPR~\citep{xiong2024ipr}{,} \\ AgentRefine~\citep{fu2025agentrefine}{,} Agent-R~\citep{yuan2025agentr};
                        }
                        ]
                    ]
                ]
                [
                    User Awareness (\S \ref{sec:interactivity}), ver
                    [
                        User State \\ Tracking % intent tracking
                        [
                        IC-DST~\citep{hu2022icdst}{,} LDST~\citep{feng2023ldst}{,} \\ \cite{hudecek-dusek-2023-are_llms_tod}{,} FNCTOD~\citep{li2024fnctod}{,} \\ \cite{king-flanigan-2024-unsupervised}{,} CoALM~\citep{acikgoz2025singlemodelmastermultiturn};\\ INTENT-SIM~\citep{zhang2023clarify}{,} Intention-in-Interaction~\citep{qian2024tell}{,} \\ AwN~\citep{wang2024learning}{,}
                        STaR-GATE~\citep{andukuri2024star}{,}  \\ AskToAct~\citep{zhang2025asktoact}           
                        ]
                    ]
                    [
                        Personalization \\ \& Persona
                        [
                        {
                        BeCand~\citep{lim2023beyond}{,} PAA~\citep{huang2023personalized}{,} \\ CharacterChat~\citep{tu2023characterchat}
                        }
                        ]
                    ]
                    [
                        Emotion \\ \& Sentiment
                        [
                        {
                        EmpatheticDialogues~\citep{rashkin-etal-2019-towards} ESConv~\citep{liu2021towards}{,} \\ D4~\citep{yao-etal-2022-d4}{,} RR~\citep{fu-etal-2023-reasoning} \\
                        }
                        ]
                    ]
                ]
                % [
                %     Continuous Learning \\ \& Adaptation (\S \ref{sec:interactivity}), ver
                %     [
                %         Online Learning \\ \& RL
                %         [
                %         TODO                        ]
                %     ]
                %     [
                %         Generalizability \\ \& Domain \\ Adaptation
                %         [
                %         {
                %         TODO
                %         }
                %         ]
                %     ]
                % ]
            ]
        \end{forest}
    }

==> sections/tables/taxonomy-ver5.tex <==
\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=6.0em,font=\small,}{},
            where level=2{text width=7.0em,font=\small,}{},
            where level=3{last level, text width=24em,font=\small,}{},
            [
                Conversational Agents, ver
                [
                    Control (\S \ref{sec:core_components}), ver
                    [
                        Complex \\ Reasoning, ver % Planning should be there
                        [
                        CoT~\citep{wei2022chain}{,} SC~\citep{wang2022sc}{,} \\ Self-Refine~\citep{madaan2023sr}{,} Reflexion~\citep{shinn2023reflexion}{,} \\ToT~\citep{yao2023tree}{,} Cue-CoT~\citep{wang-etal-2023-cue}{,} ReSpAct~\citep{dongre2024respact}
                        ]
                    ]
                    [
                        Tool Usage, ver % Knowledge Injection, RAG: Previously they use Information Retrievel, Rag now tools.
                        [
                        TALM~\citep{parisi2022talm}{,} Toolformer~\citep{schick2023toolformer}{,} \\ ToolAlpaca~\citep{tang2023toolalpaca}{,} Agent-Tuning~\citep{zeng2024agenttuning}{,} \\ Agent-Flan~\citep{chen2024agentflan}{,} FNC-TOD~\citep{li2024fnctod}{,} \\ ToolAce~\citep{liu2025toolace}{,} Hammer~\citep{lin2025hammer};\\
                        AppBench~\citep{wang-etal-2024-appbench}
                        ]
                    ]

                    [
                        Policy Following, ver % construct reward, faciliate it is as rubrics
                        [
                        {
                        SGPTOD~\citep{zhang2023sgptod}{,} \cite{hudecek-dusek-2023-are_llms_tod}{,} \\ FlowBench~\citep{xiao2024flowbench}{,}  AutoTOD~\citep{xu2024autotod}{,} \\
                        }
                        ]
                    ]
                ]
                [   Monitor (\S \ref{sec:interactivity}), ver
                    [
                        Self Awareness, ver
                        [
                            {
                            \textbf{Self-Impose Capability:}
                            SMARTAgent~\citep{qian2025smart}{,}\\ MeCo~\citep{li2025adaptive}, KnowSelf~\citep{qiao2025agentic} \\ \\
                            \textbf{Self-Correction:}
                            Self-Refine~\citep{madaan2023sr}{,}  \\ Reflexion~\citep{shinn2023reflexion}{,} ETO~\citep{song2024eto}{,} IPR~\citep{xiong2024ipr}{,} \\ AgentRefine~\citep{fu2025agentrefine}{,} Agent-R~\citep{yuan2025agentr};
                            }
                        ]
                    ]
                    [
                        User Awareness, ver
                        [
                            {
                            \textbf{User State Tracking} % intent tracking
                            IC-DST~\citep{hu2022icdst}{,} LDST~\citep{feng2023ldst}{,} \\ \cite{hudecek-dusek-2023-are_llms_tod}{,} FNCTOD~\citep{li2024fnctod}{,} \\ \cite{king-flanigan-2024-unsupervised}{,} CoALM~\citep{acikgoz2025singlemodelmastermultiturn};\\ INTENT-SIM~\citep{zhang2023clarify}{,} Intention-in-Interaction~\citep{qian2024tell}{,} \\ AwN~\citep{wang2024learning}{,}
                            STaR-GATE~\citep{andukuri2024star}{,}  \\ AskToAct~\citep{zhang2025asktoact}  \\ \\
                            \textbf{Personalization and Persona}
                            BeCand~\citep{lim2023beyond}{,} PAA~\citep{huang2023personalized}{,} \\ CharacterChat~\citep{tu2023characterchat} \\ \\
                            \textbf{Emotion and Sentiment}
                            EmpatheticDialogues~\citep{rashkin-etal-2019-towards} ESConv~\citep{liu2021towards}{,} \\ D4~\citep{yao-etal-2022-d4}{,} RR~\citep{fu-etal-2023-reasoning};
                            }
                        ]
                    ]
                ]
            ]
        \end{forest}
    }

==> sections/tables/taxonomy-ver6.tex <==
\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=3.5em,font=\tiny,}{},
            where level=2{text width=6.0em,font=\tiny,}{},
            where level=3{last level, text width=22.5em,font=\tiny,}{},
            [
                Conversational Agents, ver
                [
                    Reasoning \\ (\S \ref{sec:reason})
                    [
                        General Reasoning
                        [
                        CoT~\citep{wei2022chain}{,} SC~\citep{wang2022sc}{,} \\ Self-Refine~\citep{madaan2023sr}{,} Cue-CoT~\citep{wang-etal-2023-cue}{,}\\
                        ]
                    ]
                    [
                        Agentic Prompting
                        [
                        ReAct~\citep{yao2023reactsynergizingreasoningacting-react}{,} ToT~\citep{yao2023tree}{,}\\ Reflexion~\citep{shinn2023reflexion}{,} ReSpAct~\citep{dongre2024respact}{,} \\ 
                        ]
                    ]
                    [
                        Auto-Prompting
                        [
                        DSPy~\citep{khattab2023dspy}{,} TextGrad~\citep{yuksekgonul2024textgrad} \\
                        ]
                    ]
                ]
                [
                    Monitor \\ (\S \ref{sec:monitor})
                    [
                        Self Awareness
                        [
                        {
                        \textbf{Self-Impose Capability} SMARTAgent~\citep{qian2025smart}{,} MeCo~\citep{li2025adaptive}, \\ KnowSelf~\citep{qiao2025agentic}{,} Self-DC~\citep{wang2025selfdcreasonactself} \\
                        \textbf{Self-Correction}
                        Self-Refine~\citep{madaan2023sr}{,}  Reflexion~\citep{shinn2023reflexion}{,} \\ ETO~\citep{song2024eto}{,} IPR~\citep{xiong2024ipr}{,} AgentRefine~\citep{fu2025agentrefine}{,} \\ Agent-R~\citep{yuan2025agentr};
                        }
                        ]
                    ]
                    [
                        User \& Interaction \\ Monitoring
                        [
                        \textbf{User State Tracking} IC-DST~\citep{hu2022icdst}{,} LDST~\citep{feng2023ldst}{,} \\ \cite{hudecek-dusek-2023-are_llms_tod}{,} FNCTOD~\citep{li2024fnctod}{,} \\ \cite{king-flanigan-2024-unsupervised}{,} CoALM~\citep{acikgoz2025singlemodelmastermultiturn}\\ INTENT-SIM~\citep{zhang2023clarify}{,} Intention-in-Interaction~\citep{qian2024tell}{,} \\ AwN~\citep{wang2024learning}{,}
                        STaR-GATE~\citep{andukuri2024star}{,}  \\ AskToAct~\citep{zhang2025asktoact} \\
                        \textbf{Personalization and Persona}
                        BeCand~\citep{lim2023beyond}{,} PAA~\citep{huang2023personalized}{,} \\ CharacterChat~\citep{tu2023characterchat} \\
                        \textbf{Emotion and Sentiment}
                        EmpatheticDialogues~\citep{rashkin-etal-2019-towards}{,}\\ ESConv~\citep{liu2021towards}{,} D4~\citep{yao-etal-2022-d4}{,} RR~\citep{fu-etal-2023-reasoning}
                        ]
                    ]
                ]
                [
                    Control \\ (\S \ref{sec:control})
                    [
                        Tool Utilization
                        [
                        \textbf{Tool Creation} TALM~\citep{parisi2022talm}{,} CREATOR~\citep{qian2023creator}{,} \\ LATM~\citep{cai2024latm} \\
                        \textbf{Tool Selection} Toolformer~\citep{schick2023toolformer}{,} ToolAlpaca~\citep{tang2023toolalpaca}{,} \\ Gorilla~\citep{patil2023gorilla}{,} xLAM~\citep{zhang2024xlam}{,} Hammer~\citep{lin2025hammer} \\
                        \textbf{Tool Execution} Agent-Tuning~\citep{zeng2024agenttuning}{,} Agent-Flan~\citep{chen2024agentflan}{,} \\ FNCTOD~\citep{li2024fnctod}{,} ToolAce~\citep{liu2025toolace}{,} AppBench~\citep{wang-etal-2024-appbench} \\ 
                        ]
                    ]
                    [
                        Policy Following
                        [
                        SGPTOD~\citep{zhang2023sgptod}{,} \cite{hudecek-dusek-2023-are_llms_tod}{,} \\ FlowBench~\citep{xiao2024flowbench}{,} AutoTOD~\citep{xu2024autotod}{,} \\
                        ]
                    ]
                ]
            ]
        \end{forest}
    }

==> sections/tables/taxonomy-ver7.tex <==
\resizebox{\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=orange,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
                last level/.style={fill=orange!2}, % Define style for last level
            },
            where level=1{text width=3.0em,font=\tiny,}{},
            where level=2{text width=5.3em,font=\tiny,}{},
            where level=3{last level, text width=25.8em,font=\tiny,}{},
            [
                \textbf{Conversational Agents}, ver
                [
                    \textbf{Reasoning }\\ (\S \ref{sec:reason})
                    [
                        \textbf{General Reasoning} \\ (\S \ref{sec:general-reasoning})
                        [
                        CoT~\citep{wei2022chain}{,} SC~\citep{wang2022sc}{,} Least-to-Most~\citep{zhou2023leasttomost}{,} \\ ZeroCoT~\citep{kojima2022zerocot}{,} PoT~\citep{chen2023pot}{,} PAL~\citep{gao2023pal}{,} \\ Self-Refine~\citep{madaan2023sr}{,} GoT~\citep{wang-etal-2023-cue}{,} Cue-CoT~\citep{wang-etal-2023-cue}\\
                        ]
                    ]
                    [
                        \textbf{Agentic Reasoning} \\ (\S \ref{sec:agentic-reasoning})
                        [
                        ReAct~\citep{yao2023reactsynergizingreasoningacting-react}{,} ART~\citep{paranjape2023art}{,} Reflexion~\citep{shinn2023reflexion}{,}\\ ToT~\citep{yao2023tree}{,}  MultiTool-CoT~\citep{inaba2023multitool}{,} ChatCoT~\citep{chen2023chatcot}{,} \\ LATS~\citep{zhou2023lats}{,} ToolChain*~\citep{zhuang2023toolchain}{,} ReSpAct~\citep{dongre2024respact} \\ 
                        ]
                    ]
                ]
                [
                    \textbf{Monitor} \\ (\S \ref{sec:monitor})
                    [
                        \textbf{Self-Awareness} \\ (\S \ref{sec:self-awareness})
                        [
                        {
                        \textbf{Self-Impose Capability}  \cite{mielke2022reducingconvagentcalibration}{,} SelfAware~\citep{yin2023selfaware}{,}  \\ KUQ~\citep{amayuelas2024kuq}{,} Idk~\citep{cheng2024idk}{,} Self-DC~\citep{wang2025selfdcreasonactself}{,} \\ SMARTAgent~\citep{qian2025smart}{,} MeCo~\citep{li2025adaptive}, KnowSelf~\citep{qiao2025agentic} \\
                        \textbf{Self-Correction}
                        Self-Refine~\citep{madaan2023sr}{,} LVSBS~\citep{lightman2024lvsbs}{,} \\ Reflexion~\citep{shinn2023reflexion}{,} RAP~\cite{hao2023rap}{,} ETO~\citep{song2024eto}{,} \\ IPR~\citep{xiong2024ipr}{,} AgentRefine~\citep{fu2025agentrefine}{,} Agent-R~\citep{yuan2025agentr}
                        }
                        ]
                    ]
                    [
                        \textbf{User \& Interaction} \\ \textbf{Monitoring} \\ (\S \ref{sec:user-monitoring})
                        [
                        \textbf{User State Tracking} EMD~\citep{wang-etal-2021-fast}{,} IC-DST~\citep{hu2022icdst}{,} \cite{heck2023chatgptzeroshotdst}{,} \\  \cite{hudecek-dusek-2023-are_llms_tod}{,} InstructTODS~\citep{chung2023instructtods}{,} LDST~\citep{feng2023ldst}{,} \\ INTENT-SIM~\citep{zhang2023clarify}{,}  FNCTOD~\citep{li2024fnctod}{,} AwN~\citep{wang2024learning}{,} \\ Intention-in-Interaction~\citep{qian2024tell}{,} STaR-GATE~\citep{andukuri2024star}{,} \\ \cite{king-flanigan-2024-unsupervised}{,}  CoALM~\citep{acikgoz2025singlemodelmastermultiturn}{,} AskToAct~\citep{zhang2025asktoact} \\
                        \textbf{Personalization and Persona}
                         PERSONA-CHAT~\citep{zhang2018personalizingdialogue}{,} PAA~\citep{huang2023personalized}{,} \\ LaMP~\citep{salemi2024lamp}{,} Generative Agents~\citep{generative_agents}{,} BeCand~\citep{lim2023beyond}{,} \\ CharacterChat~\citep{tu2023characterchat}{,} OPPU~\citep{tan2024oppu}{,} Per-Pcs~\citep{tan2024perpcs} \\
                        \textbf{Emotion and Sentiment}
                        EmpatheticDialogues~\citep{rashkin-etal-2019-towards}{,} ESConv~\citep{liu2021towards}{,} \\ D4~\citep{yao-etal-2022-d4}{,} \cite{zhao2023chatgptemotion}{,} Cue-CoT~\citep{wang-etal-2023-cue}{,} RR~\citep{fu-etal-2023-reasoning}
                        ]
                    ]
                ]
                [
                    \textbf{Control} \\ (\S \ref{sec:control})
                    [
                        \textbf{Tool Utilization} \\ (\S \ref{sec:tool_utilization})
                        [
                        \textbf{Tool Selection} TALM~\citep{parisi2022talm}{,} Toolformer~\citep{schick2023toolformer}{,} \\ Gorilla~\citep{patil2023gorilla}{,} CREATOR~\citep{qian2023creator}{,} LATM~\citep{cai2024latm}{,} \\ Granite~\citep{abdelaziz2024granite}{,} xLAM~\citep{zhang2024xlam}{,} Hammer~\citep{lin2025hammer}{,} \\
                        \textbf{Tool Execution} ToolkenGPT~\citep{hao2023toolkengpt}{,} HuggingGPT~\citep{shen2023hugginggpt}{,} \\ ToolAlpaca~\citep{tang2023toolalpaca}{,} ToolLLM~\citep{qin2024toolllm}{,} Agent-Tuning~\citep{zeng2024agenttuning}{,} \\ FireAct~\citep{chen2023fireact}{,} CodeAct~\citep{wang2024codeact}{,} Agent-Flan~\citep{chen2024agentflan}{,} \\ FNCTOD~\citep{li2024fnctod}{,} ToolAce~\citep{liu2025toolace}{,} CoALM~\citep{acikgoz2025singlemodelmastermultiturn}\\ 
                        ]%AppBench~\citep{wang-etal-2024-appbench} 
                    ]
                    [
                        \textbf{Policy Learning} \\ \& \textbf{Following} \\ (\S \ref{sec:policy_following})
                        [
                         \cite{wen-etal-2017-network}{,} \cite{bing2017policy}{,} Deep Dyna-Q~\citep{peng-etal-2018-deep}{,} \\  DDPT~\citep{geishauser-etal-2022-dynamic}{,} SGPTOD~\citep{zhang2023sgptod}{,} \cite{hudecek-dusek-2023-are_llms_tod}{,} \\ $\tau$-Bench~\citep{Yao2024tau}{,} FlowBench~\citep{xiao2024flowbench}{,} AutoTOD~\citep{xu2024autotod} \\
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
